Breadboarding the European Moon Rover System: discussion and results of the analogue field test campaign

This document compiles results obtained from the test campaign of the European Moon Rover System (EMRS) project. The test campaign, conducted at the Planetary Exploration Lab of DLR in Wessling, aimed to understand the scope of the EMRS breadboard design, its strengths, and the benefits of the modular design. The discussion of test results is based on rover traversal analyses, robustness assessments, wheel deflection analyses, and the overall transportation cost of the rover. This not only enables the comparison of locomotion modes on lunar regolith but also facilitates critical decision-making in the design of future lunar missions.

==> review1_comments/reviewer2_comments.tex <==
This paper describes the testing of a novel prototype rover
for the future EMRS. This rover has 4 wheels with 2 motors
each, so its configuration allows the execution of
Ackermann, Skid-steering, Crabbing and Point-Turn, granting
it a high range of mobility capabilities. Moreover, this
prototype is equipped with wheels that can passively adapt
to the shape of negotiable obstacles, so the traversability
is enhanced. The purpose of the test results presented in
this paper focus on studying the mobility skills of this
prototype rover through three types of test: a comparative
between different locomotion modes, the deflection of the
wheels when going over an obstacle and the cost of
transport when traversing slopes.

I find the concept of these tests interesting from the
point of view of them being a first step towards developing
the mobility system of the future EMRS. However, it is not
clear to me how the presented solution complies with the
requirements for future Moon missions. I do not see in the
text any direct link between these requirements (speed?
obstacles to negotiate? max slopes to traverse?) and the
demonstrated mobility skills, yet in the text it is
thoroughly claimed that this prototype already validates
such requirements.

I have collected a series of notes organized by page. I
consider addressing them would notably enhance the quality
of the paper and increase its clarity.

Page 1:

- Take this please just as a suggestion. Fig.1 could use a
picture of the rover in a real setup instead of this
montage. For example, in reference [8] I see there is a
similar image of the experiment inside a facility, that
would be more formal and informative.

- I do not understand the reason for adding [7] at the end
of the first paragraph (publication about a robotic
software for rover-rover and rover-astronaut interaction)

- In 2nd paragraph, in which sense the rover design focus
is modularity? Maybe elaborate or add a reference that
supports this statement, I find it more times over the
paper but it is not clear to me why.

- Typo: after DLR facilities, add a space after the comma.

- I cannot find Reference [9]. Is it a written publication
(paper, book chapter...) or maybe a webpage?

Page 2:

- How will EMRS adapt to the different proposed missions
described in Section III? I assume these missions will
entail different requirements, maybe a bit more of
elaboration (or a reference further explaining this) would
be good.

- In Section IV, "The successful development of the EMRS
breadboard validates the modular mobility concept for a
multipurpose rover", how? I have no clear idea why this
mobility is "modular" (what is the difference with respect
to other systems also equipped with 4 steerable wheels?)

- By the end of Section IV, what are the COTS and space
components of this rover, which are claimed to meet design
requirements? And what are these design requirements?

Page 3:

- What is the motion capture system used for the
experiments? Vicon? Optitrack? Other?

- Typo: These tests were mainly conducted to prove [...]
(not to proof)

- Typo: [...] as well as to test the on-board [...] (there
is a "to" missing

- Typo (by the end of the page): The loss of wheel motion
[...] (instead of "the lost of")

Page 4:

- Is there more information anywhere about these wheels? I
guess given the images that they are designed to be
flexible but I do not see this explicitly stated in the
text. A brief description or reference would be appreciated
to understand better their role in the mobility system.

- What is the shape of the obstacle used for the wheel
deflection test?

- How do you define deflection here? Is it the volume
estimated (colored in magenta in the figures) divided by
the total volume? If so, adding an equation would add
clarity.

- The X-axis of Fig. 6 says "Iter", is it the frame number?
What is the framerate used to record the video?

- Adding legends to Fig. 6 would be useful.

Page 5:

- Is 6.5\% of deflection an EMRS requirement? (number found
at the end of subsection C)

- What was the speed of the rover during the COT test?
Maybe very low speed could cause this increase in motor
energy consumption when driving horizontally, which would
be solved by driving faster.

- Was the speed measured using wheel odometry or using the
motion capture system? Using the second would be key here
as the slippage could affect the actual speed of the rover
or the energy consumption (in other words, with high slope
maybe the rover would have to command the wheels to rotate
faster to compensate for such slippage, thus increasing the
energy consumption).

- In the Discussion section: "Notably, the rover has
surpassed the requirements in executing these locomotion
modes, underscoring in robust performance. This achievement
is attributed to the modular design, which enables
adaptability and versatility in locomotion". Which
requirements? More than a performance analysis (which would
entail a thorough analysis on the rover motion -steering
angles, XY position error with respect to commands...) I
see the presented test as a validation to check the rover
is indeed capable to execute many different locomotion
modes. Why the design is categorized as "modular"? (similar
question to previous comment of mine) 
